Post-Hoc Answer Attribution for Grounded and Trustworthy Long Document Comprehension: Task, Insights, and Challenges

Attributing answer text to its source document for information-seeking questions is crucial for building trustworthy, reliable, and accountable systems. We formulate a new task of post-hoc answer attribution for long document comprehension (LDC). Owing to the lack of long-form abstractive and information-seeking LDC datasets, we refactor existing datasets to assess the strengths and weaknesses of existing retrieval-based and proposed answer decomposition and textual entailment-based optimal selection attribution systems for this task. We throw light on the limitations of existing datasets and the need for datasets to assess the actual performance of systems on this task.

==> sections/02_task_definition.tex <==
% \section{Answer Attribution Task Definition} \label{sec:task_definition}
% We characterize the task of answer attribution for long document comprehension as: given
% a query $Q$, $n$ text snippets (sentences) $S=s_1, \dots, s_n$ from document $D$, and an answer (either, generated from a system or ground-truth) to query $Q$, the goal is to identify supporting text snippets (namely, attributions) $s_i\in S$ for each sentence $a_i\in A=a_1, \dots, a_m$. Each sentence may be attributed to multiple text snippets.




==> sections/07related.tex <==
\section{Related Work}
\paragraph{Claim Verification or summary-source alignment}
\paragraph{Evidence Retrieval}
- at an answer level
- mostly used as an auxiliary task, answer is generated along with the evidence
\paragraph{Attributability}
Question Answering
- open-domain 
- short or one word answers
- answer is generated along with citations

Rashkin et al. (2023) formalize
an attributable statement to identified sources such
that it can be entailed from some underlying corpus by a generic hearer. Thus, attributability is
a specific form of explainability within the constraints of a given source. WebGPT (Nakano et al.,
2021) and GopherCite (Menick et al., 2022) are
two recent closed-source models that are capable
of generating references to their supporting evidence. From the data perspective, several QA
datasets (Geva et al., 2021; Bohnet et al., 2022)
provide pointers to text snippets supporting the
gold answer. Moreover, two recent works (Liu
et al., 2023a; Gao et al., 2023) focus on verifying
citations in generated text based on a given set of
quotes, which closely aligns with our objective in
this paper. Specifically, Liu et al. (2023a) focus on
closed-source proprietary search engines, whereas
our goal is to use publicly available data to allow
for building open-source end-to-end search models. Similarly, ALCE (Gao et al., 2023), a concurrent work to HAGRID, shares a similar goal,
albeit with two notable differences. First, Gao
et al. (2023) derive questions from QA datasets


Answer attribution is a new field of research owing to the recent advancement in Generative AI and introduction of large language models. The task of answer attribution is related to the task of claim verification \citep{wadden-etal-2020-fact,glockner2020you,chen2023complex,kamoi2023wice} wherein a claim can be either supported or refuted by a passage or document. Recent approaches to claim verification [2,4] decompose claims into subclaims to find support for each sub-claim and then combine the predictions to get a prediction for overall claim. Other works include evidence extraction for question answering~\citep{wang-etal-2019-evidence} and attributed question answering~\citep{bohnet2022attributed}. However \citet{wang-etal-2019-evidence} considers extractive MCQ type answers while our focus is on long-form abstractive answers. On the other hand, \citet{bohnet} considers one passage per answer as attribution whereas our focus is on more fine-grained attribution. Another line of works include Question answering LLM chains (stuff, map/reduce, or refine) that request the indication of sources that have been used for answering during answer generation. A LLM prompt may look like this: """Given the following extracted parts of a long document and a question, create a final answer with references ("SOURCES").""" The attributions provided in this style have several disadvantages (a) only assigned to the overall answer (not assigned to answer parts), (b) no control over selection or ranking (e.g., the number of attributions cannot be adjusted, relevance is unknown, experience not customizable), (c) additional related attributions need to be provided via separate methods, and (d) answer quality/style is negatively impacted.


Methods

With the rapid adaptation of large language models, a few different classes of systems have been proposed for generating attributions for the responses they produce. The first class of systems is vanilla LLM prompting (Tay et al., 2022; Weller et al., 2023), where LLMs such as GPT-4 (OpenAI, 2023) are prompted to return attributions (in the form of titles of references, optionally accompanied with URLs) along with their answers. Since these systems are not explicitly trained to produce attributions, they can often hallucinate the references they provide (Agrawal et al., 2023). Another class of systems is retrieve-and-read systems (Guu et al., 2020; Borgeaud et al., 2022; Izacard et al., 2022), which first retrieve evidence relevant for a query, and then generate an answer based on the retrieved evidence. These systems are sometimes trained on demonstrations of humans browsing for information (Nakano et al., 2021; Thoppilan et al., 2022; Menick et al., 2022), which allows them to jointly generate answers and citations. Finally, post-hoc retrieval (Gao et al., 2023; He et al., 2022) involves retrieving attributions after answering a query using both the query and response for retrieval, and optionally revising the answer based on the attribution. For sampling responses, we consider all three classes of systems described above.


analysis

Prior work has conducted
analysis of attributions produced by systems in
response to queries from existing NLP datasets
(Rashkin et al., 2021; Bohnet et al., 2022; Dziri
et al., 2022; Liu et al., 2023; Muller et al., 2023).
Notably, Rashkin et al. (2021) propose the framework of Attributable to Identified Sources (AIS)
for performing human evaluation of attributions. Analysis from these works suggests that systems
are still far from providing precise attributions with
sufficient recall for all citeworthy statements. In
our work, we recognize that this is problematic in
specific domains where attribution precision and
recall are both critical.
Automatic methods to measure attribution have
also been explored. Briefly, attribution has been
automatically measured through the use of textual
entailment models (Bohnet et al., 2022; Yue et al.,
2023), by checking the consistency of answers produced to the same question using the evidence or
the response (Wang et al., 2020) and prompting
LLMs and finetuning LLMs on tasks such as NLI
relevant for judging attributions (Yue et al., 2023).
Previous efforts at collecting gold attribution data have been conducted by repurposing
Wikipedia citations (Kamoi et al., 2023; Petroni
et al., 2022), or existing datasets like Natural Questions (Bohnet et al., 2022; Kwiatkowski et al.,
2019), and relying on large-scale human annotation (Chen et al., 2022; Dziri et al., 2022; Kamalloo
et al., 2023). We note that with regards to the information needs of experts, this data can be restricting
in terms of the accompanying corpus, and contain
limited complexity when it comes to expert-curated
content (for instance, experts are likely to use and
trust sources other than Wikipedia).
